Towards Real-world Human Behavior Simulation: Benchmarking Large Language Models on Long-horizon, Cross-scenario, Heterogeneous Behavior Traces

The emergence of Large Language Models (LLMs) has illuminated the potential for a general-purpose user simulator. However, existing benchmarks remain constrained to isolated scenarios, narrow action spaces, or synthetic data, failing to capture the holistic nature of authentic human behavior. To bridge this gap, we introduce OmniBehavior, the first predictive user simulation benchmark constructed entirely from real-world data, integrating long-horizon, cross-scenario, and heterogeneous behavioral patterns into a unified framework. Based on this benchmark, we first provide empirical evidence that previous datasets with isolated scenarios suffer from tunnel vision, whereas real-world decision-making relies on long-term, cross-scenario causal chains. Extensive evaluations of state-of-the-art LLMs reveal that current models struggle to accurately predict these complex behaviors, with performance plateauing even as context windows expand. Crucially, a systematic comparison between simulated and authentic behaviors uncovers a fundamental structural bias: LLMs tend to converge towards a positive average person, exhibiting hyper-activity, persona homogenization, and a utopian bias. This results in the loss of individual differences and long-tail behaviors, highlighting critical directions for future high-fidelity simulation research.

==> macros.tex <==
\PassOptionsToPackage{numbers, compress}{natbib}



\usepackage[final]{neurips_2025}


\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage{hyperref}       %
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{xcolor}         %

\usepackage{abbrv}

\usepackage{amsmath}
\usepackage{multirow}
\usepackage{wrapfig}
\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage[export]{adjustbox}
\usepackage[capitalize]{cleveref}
\crefname{figure}{Figure}{Figures}

\usepackage[most]{tcolorbox}
\definecolor{prompt}{HTML}{5f84e4}
\definecolor{img}{HTML}{820100}

\usepackage{listings}
\lstset{%
basicstyle={\scriptsize\ttfamily},
numberstyle=\scriptsize,
showstringspaces=false,
language=Python,
keywordstyle=\color{blue},
mathescape=true,
escapeinside={<}{>},
aboveskip=0pt,
belowskip=0pt,
}

\def\method{\textsc{SpatialLM}\xspace}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\ZH}[1]{\textcolor{orange}{[Zihan: #1]}}
\newcommand{\MB}[1]{\textcolor{teal}{[Mubin: #1]}}
\newcommand{\FD}[1]{\textcolor{purple}{[Fandong: #1]}}

\newcommand{\G}{\mathcal{G}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\D}{\mathbf{D}}
\renewcommand{\L}{\mathbf{L}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\Z}{\mathcal{Z}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\I}{\mathcal{I}}
\renewcommand{\O}{\mathbf{O}}

\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\c}{\mathbf{c}}
\newcommand{\n}{\mathbf{n}}
\renewcommand{\l}{\mathbf{l}}
\renewcommand{\d}{\mathbf{d}}
\renewcommand{\t}{\mathbf{t}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\q}{\mathbf{q}}
\renewcommand{\u}{\mathbf{u}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\w}{\mathbf{w}}
\renewcommand{\a}{\mathbf{a}}

\renewcommand\tabularxcolumn[1]{m{#1}}%
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\definecolor{seatings}{HTML}{39e133}
\definecolor{beddings}{HTML}{9d2bf5}
\definecolor{cabinetry}{HTML}{fd8630}
\definecolor{tables}{HTML}{33ebf7}
\definecolor{kitchen_appliances}{HTML}{3e6271}
\definecolor{bathroom_fixtures}{HTML}{f786e1}
\definecolor{lighting}{HTML}{c9f659}
\definecolor{decoration}{HTML}{e92c7e}
\definecolor{electronics}{HTML}{5485fe}
\definecolor{others}{HTML}{a4cbdb}

